Guided Fine-Tuning for Large-Scale Material Transfer

We present a method to transfer the appearance of one or a few exemplar SVBRDFs to a target image representing similar materials. Our solution is extremely simple: we fine-tune a deep appearance-capture network on the provided exemplars, such that it learns to extract similar SVBRDF values from the target image. We introduce two novel material capture and design workflows that demonstrate the strength of this simple approach. Our first workflow allows to produce plausible SVBRDFs of large-scale objects from only a few pictures. Specifically, users only need take a single picture of a large surface and a few close-up flash pictures of some of its details. We use existing methods to extract SVBRDF parameters from the close-ups, and our method to transfer these parameters to the entire surface, enabling the lightweight capture of surfaces several meters wide such as murals, floors and furniture. In our second workflow, we provide a powerful way for users to create large SVBRDFs from internet pictures by transferring the appearance of existing, pre-designed SVBRDFs. By selecting different exemplars, users can control the materials assigned to the target image, greatly enhancing the creative possibilities offered by deep appearance capture.

==> 4_Processing.tex <==
\section{Process}
\label{sec:process}



==> 6_training.tex <==
\subsection{Training}
\label{sec:training}

%We train our network end to end and choose to let the final loss gradient propagate to the material encoder, rather than enforce an intermediate loss. This ensure that the encoder is trained to extract parameters from the material examples with the only objective to help the main network inference.

We trained our deep network with synthetic SVBRDFs \cite{Substance} that provide ground truth supervision for each parameter map. We rely on the same set of training SVBRDFs as Deschaintre et al.~\shortcite{Deschaintre18}, except that we render them at a higher resolution of $2048 \times 2048$ pixels. At each training step, a unique material is created by mixing two of these pre-computed SVBRDFs. We then extract between $1$ and $3$ patches of $256 \times 256$ pixels to form the SVBRDF exemplars. Finally, we extract a large crop to serve as the input image, which we resize to $512 \times 512$ pixels to be fed to the network. We vary the size of this crop between $512 \times 512$ and $1024 \times 1024$ pixels, such that the input image and SVBRDF exemplars contain features of different scales. Similarly to Deschaintre et al.~\shortcite{Deschaintre19}, we perform all these processing steps at training time in TensorFlow \cite{tensorflow2015} to reduce storage and data transfer.

%We use a new dataset of materials generated in 2048x2048, using the same set of substances \cite{Substance} as Deschaintre et al.~\shortcite{Deschaintre18}. At each step, we randomly mix 2 materials together and randomly crop an image with a resolution between 512x512 and 1024x1024. This crop is then resized to 512x512 and rendered to be used as the HD image crop input. We use this resize approach to generate different scales of input image crop and material examples. The examples are randomly extracted from the 2048x2048 mixed material in the form of 256x256 material patches. All of these steps are taken in tensorflow, in a similar manner to Deschaintre et al.~\shortcite{Deschaintre19}. This allows us to avoid huge storage and disk i/o costs given the dataset high resolution, but also flexibility in the generation of the training inputs.

%The end to end training is done on a GV100 or two 1080TI. 
We trained the network for $700~000$ steps to obtain the results shown in this paper and supplemental materials, which took around 6 days on a GV100 graphics card.


%\begin{figure*}
%  \centering
%    \includegraphics[width=\textwidth]{img/temp_figure}
%     \caption{A normal map just stitched together and a normal map smoothly stitched.}
%     \label{fig:withoutwithSmoothing}
%\end{figure*}
